Widget2Code: From Visual Widgets to UI Code via Multimodal LLMs

User interface to code (UI2Code) aims to generate executable code that can faithfully reconstruct a given input UI. Prior work focuses largely on web pages and mobile screens, leaving app widgets underexplored. Unlike web or mobile UIs with rich hierarchical context, widgets are compact, context-free micro-interfaces that summarize key information through dense layouts and iconography under strict spatial constraints. Moreover, while (image, code) pairs are widely available for web or mobile UIs, widget designs are proprietary and lack accessible markup. We formalize this setting as the Widget-to-Code (Widget2Code) and introduce an image-only widget benchmark with fine-grained, multi-dimensional evaluation metrics. Benchmarking shows that although generalized multimodal large language models (MLLMs) outperform specialized UI2Code methods, they still produce unreliable and visually inconsistent code. To address these limitations, we develop a baseline that jointly advances perceptual understanding and structured code generation. At the perceptual level, we follow widget design principles to assemble atomic components into complete layouts, equipped with icon retrieval and reusable visualization modules. At the system level, we design an end-to-end infrastructure, WidgetFactory, which includes a framework-agnostic widget-tailored domain-specific language (WidgetDSL) and a compiler that translates it into multiple front-end implementations (e.g., React, HTML/CSS). An adaptive rendering module further refines spatial dimensions to satisfy compactness constraints. Together, these contributions substantially enhance visual fidelity, establishing a strong baseline and unified infrastructure for future Widget2Code research.

==> sec/Algo_Fig_Tab/AutoResize.tex <==
\begin{algorithm}[t]
\caption{Aspect-Ratio-Aware Widget Auto-Resize}
\label{alg:autoresize}
\begin{algorithmic}[1]
\REQUIRE Widget element $E$, target aspect ratio $r$
\ENSURE Optimal dimensions $(w^*, h^*)$ satisfying content fit and aspect ratio
\STATE $w_0 \leftarrow \text{GetNaturalWidth}(E)$
\STATE $w_{\text{init}} \leftarrow \max(40, w_0)$, $h_{\text{init}} \leftarrow w_{\text{init}} / r$
\STATE $\text{ApplySize}(E, w_{\text{init}}, h_{\text{init}})$
\STATE $f_{\text{init}} \leftarrow \text{CheckFit}(E)$
\IF{$f_{\text{init}} = \text{true}$}
    \STATE $w_l \leftarrow 40$, $w_h \leftarrow w_{\text{init}}$
    \WHILE{$w_h - w_l > 1$}
        \STATE $w_m \leftarrow \lfloor (w_l + w_h) / 2 \rfloor$, $h_m \leftarrow w_m / r$
        \STATE $\text{ApplySize}(E, w_m, h_m)$
        \IF{$\text{CheckFit}(E)$}
            \STATE $w^* \leftarrow w_m$, $h^* \leftarrow h_m$, $w_h \leftarrow w_m$
        \ELSE
            \STATE $w_l \leftarrow w_m$
        \ENDIF
    \ENDWHILE
\ELSE
    \STATE $w_h \leftarrow w_{\text{init}}$
    \WHILE{$\neg\text{CheckFit}(E)$ \AND $w_h < 4096$}
        \STATE $w_h \leftarrow 2w_h$, $\text{ApplySize}(E, w_h, w_h / r)$
    \ENDWHILE
    \STATE $w_l \leftarrow w_h / 2$, $w^* \leftarrow w_h$, $h^* \leftarrow w_h / r$
    \WHILE{$w_h - w_l > 1$}
        \STATE $w_m \leftarrow \lfloor (w_l + w_h) / 2 \rfloor$, $h_m \leftarrow w_m / r$
        \STATE $\text{ApplySize}(E, w_m, h_m)$
        \IF{$\text{CheckFit}(E)$}
            \STATE $w^* \leftarrow w_m$, $h^* \leftarrow h_m$, $w_h \leftarrow w_m$
        \ELSE
            \STATE $w_l \leftarrow w_m$
        \ENDIF
    \ENDWHILE
\ENDIF
\STATE \textbf{return} $(w^* + 1, h^* + 1)$
\end{algorithmic}
\end{algorithm}
\clearpage
\begin{algorithm}[t]
\caption{Widget Auto-Resize (Simplified)}
\label{alg:autoresize-simple}
\begin{algorithmic}[1]
\REQUIRE Widget element $E$, aspect ratio $r$
\ENSURE Optimal size $(w^*, h^*)$
\STATE $w \leftarrow \text{GetNaturalWidth}(E)$, $h \leftarrow w / r$
\STATE $\text{ApplySize}(E, w, h)$
\IF{$\text{CheckFit}(E)$}
    \STATE $w_l \leftarrow 40$, $w_h \leftarrow w$
\ELSE
    \WHILE{$\neg\text{CheckFit}(E)$}
        \STATE $w \leftarrow 2w$, $\text{ApplySize}(E, w, w/r)$
    \ENDWHILE
    \STATE $w_l \leftarrow w/2$, $w_h \leftarrow w$
\ENDIF
\WHILE{$w_h - w_l > 1$}
    \STATE $w_m \leftarrow (w_l + w_h) / 2$, $\text{ApplySize}(E, w_m, w_m/r)$
    \IF{$\text{CheckFit}(E)$}
        \STATE $w_h \leftarrow w_m$
    \ELSE
        \STATE $w_l \leftarrow w_m$
    \ENDIF
\ENDWHILE
\STATE \textbf{return} $(w_h, w_h/r)$
\end{algorithmic}
\end{algorithm}
